Breaking Common Sense: WHOOPS! A Vision-and-Language Benchmark of Synthetic and Compositional Images

Weird, unusual, and uncanny images pique the curiosity of observers because they challenge commonsense. For example, an image released during the 2022 world cup depicts the famous soccer stars Lionel Messi and Cristiano Ronaldo playing chess, which playfully violates our expectation that their competition should occur on the football field. Humans can easily recognize and interpret these unconventional images, but can AI models do the same? We introduce WHOOPS!, a new dataset and benchmark for visual commonsense. The dataset is comprised of purposefully commonsense-defying images created by designers using publicly-available image generation tools like Midjourney. We consider several tasks posed over the dataset. In addition to image captioning, cross-modal matching, and visual question answering, we introduce a difficult explanation generation task, where models must identify and explain why a given image is unusual. Our results show that state-of-the-art models such as GPT3 and BLIP2 still lag behind human performance on WHOOPS!. We hope our dataset will inspire the development of AI models with stronger visual commonsense reasoning abilities. Data, models and code are available at the project website: whoops-benchmark.github.io

==> figs_and_tables/fig_normal_strange.tex <==
\begin{figure}[!tb]
    \includegraphics[width=\columnwidth]{images/Fig_normal_strange.jpg}\\
    \caption{Left, weird image: a wool yarn ball (X) knocks down bowling pins (Y). Right, normal image: a bowling ball (X') knocks down bowling pins (Y).}
    \label{fig:fig_normal_strange}
\end{figure}



==> figs_and_tables/table_identification_explanation_backup.tex <==
% \begin{table*}[!htb]
% \centering
% \begin{tabular}{@{}llcccc@{}} \toprule
%                             & Task                                               & Identify && Explain  \\ \cmidrule(l){3-3} \cmidrule(l){4-6}
%                                                         &                                                 & Binary Accuracy $(\uparrow)$ 
%                                                      & Human Rating $(\uparrow)$ & Automatic Rating $(\uparrow)$ & Automatic Rating Accuracy $(\uparrow)$ \\ \midrule

% \multirow{3}{*}{End-to-end} & BLIP2 FlanT5-XXL (Zero-shot)                       &   50       & \phantom{0}0       & 0 & 100                   \\
%                             & BLIP2 FlanT5-XL (Fine-tuned)                       & 60       & 15    & 18    & 81                          \\
%                             & BLIP2 FlanT5-XXL (Fine-tuned)                      & 73       & 27    & 24    &90                         \\ \midrule
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Pipeline\\ (Zero-shot)\end{tabular}}   & Predicted Caption $\rightarrow$ GPT3               &   59       & 33    & 42    &85                         \\
%                             & Ground-truth Caption $\rightarrow$   GPT3 (Oracle) &      74    & 68  & 62    &85                         \\  \midrule
%                             & Humans                                             & 92       & 95    &                        \\ \bottomrule
% \end{tabular}
% \caption{\yonatan{expand the explanation column to three, add "Automatic Rating (arrow up)" + "Automatic Rating Accuracy (arrow up)"} Test results for Explanation-of-violation, which consists of the two subtasks of \emph{identifying} weird images and \emph{explaining} what makes them weird. Human performance far exceeds model performance on both tasks, even when an oracle image description is provided. 
% }
% \label{tab:identification_and_explanation}
% \end{table*}

\begin{table*}[!htb]
\centering
\begin{tabular}{@{}llcccc@{}}
\toprule
& Task & \multicolumn{1}{p{1.7cm}}{\centering Identify} && \multicolumn{1}{p{1.5cm}}{\centering Explain} \\
\cmidrule(l){3-3} \cmidrule(l){4-6}
& & \multicolumn{1}{p{1.9cm}}{\centering Binary Accuracy $(\uparrow)$} & \multicolumn{1}{p{1.5cm}}{\centering Human Rating $(\uparrow)$} & \multicolumn{1}{p{1.5cm}}{\centering GPT4 Rating $(\uparrow)$} & \multicolumn{1}{p{1.9cm}}{\centering GPT4 Rating Accuracy $(\uparrow)$} \\
\midrule
\multirow{3}{*}{End-to-end} & BLIP2 FlanT5-XXL (Zero-shot) & 50 & \phantom{0}0 & 12 & 88 \\
& BLIP2 FlanT5-XL (Fine-tuned) & 60 & 15 & 18 & 87 \\
& BLIP2 FlanT5-XXL (Fine-tuned) & 73 & 27 & 27 & 81 \\
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Pipeline\\ (Zero-shot)\end{tabular}} & Predicted Caption $\rightarrow$ GPT3 & 59 & 33 & 36 & 87 \\
& Ground-truth Caption $\rightarrow$ GPT3 (Oracle) & 74 & 68 & 70 & 81 \\
\midrule
& Humans & 92 & 95 & -& -\\
\midrule
\multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Post-\\Submission\\ Evaluation\end{tabular}} & Predicted Caption $\rightarrow$ GPT4 & - & - & 36 & - \\
& Ground-truth Caption $\rightarrow$ GPT4 (Oracle) & - & - & 69 & - \\
& Predicted Caption $\rightarrow$ Llama-2-7b & - & - & 36 & - \\
& Ground-truth Caption $\rightarrow$ Llama-2-7b (Oracle) & - & - & 71 & - \\
& Predicted Caption $\rightarrow$ Llama-2-13b & - & - & 36 & - \\
& Ground-truth Caption $\rightarrow$ Llama-2-13b (Oracle) & - & - & 70 & - \\
& Instruct BLIP & - & - & 31 & - \\
\bottomrule
\end{tabular}
\caption{
% \yonatan{Change 3}
Test results for Explanation-of-violation, which consists of the two subtasks of \emph{identifying} weird images and \emph{explaining} what makes them weird. Human performance far exceeds model performance on both tasks, even when an oracle image description is provided. The \emph{explaining} task involves two metrics: human rating and BART-L rating. These metrics measure the percentage of positive candidate explanations classified by humans or a fine-tuned BART-L model. The accuracy of each fine-tuned BART-L model is presented in the BART-L Rating Accuracy column.}
\label{tab:identification_and_explanation}
\end{table*}




==> sections/99A_identify.tex <==
% In this section, we evaluate how humans and models understand the simple classification task of determining whether an image contains something strange or not. To do this, we selected 100 "non-strange" images and mixed them with our dataset. Random chance would result in a 50\% accuracy rate.

% \subsection{Setup}
% For human evaluation, we hired five MTurk workers and instructed them to provide a binary classification of whether the image contained something strange or not. Full annotation guidelines and instructions are provided in Appendix A, Section~\cref{annotations}.

% For model evaluation, we used a similar setup as before, using an image captioning model injected into an instruction-based language model. This time, the instructions were to ``determine if something is strange in the image, and if so, to explain what.'' We experimented with image captions from a fine-tuned OFA image captioning model and from the ground-truth prompt used to create the image.

% \subsection{Results}
% The results of our evaluation are presented in Table 5. We found that humans were able to classify correctly in T\% of the cases, while the model only achieved accuracy in Z\% of the cases. We also found that the oracle model's predictions were much better, again suggesting the limitation of under-described image captions. Overall, these results show that humans are successful on this task, while models struggle.





==> sections/99B_what_makes_this_image_strange.tex <==
% In this section, we evaluate both humans and AI models on the task of explaining what is strange in a given image.

% \subsection{Human Evaluation}
% We first evaluate humans on this task. We crowd-source explanations and compare to the ground-truth explanations provided by the designers. 

% \paragraph{Crowd-sourcing Explanations.}
% We hired Amazon Mechanical Turk workers to provide explanations for each image in the dataset. Each worker was given an image and asked to write a single line explaining what is strange about the image. We required five annotations per image.

% \paragraph{Setup.}
% We compared the workers' explanations to the ground-truth explanation provided by the designers. To do this, we used both manual and automatic evaluation methods. For manual evaluation, we rated each explanation on whether it was the same as the ground-truth or not. An image was considered successfully annotated if it had at least 3 out of 5 explanations that were the same as the ground-truth explanation. For automatic evaluation, we experimented with three different metrics: (1) SBERT embeddings cosine similarity, (2) Q-2, an NLI-based metric for comparing two texts, and (3) an instruction-based GPT3 metric that classifies whether the explanation is the same as the ground-truth or not. We selected the best automatic metric by comparing it to the human evaluation method.


% \paragraph{Results.}
% Results are presented in Table 1. We found that in X\%, there were at least 3 out of 5 explanations that were the same as the ground-truth explanations. Overall, Y\% of the explanations were the same as the ground-truth.


% For the automatic evaluation methods, we found that the XYZ metric performed similarly to the human evaluation method, with high agreement with the ground-truth annotation and the dataset label. These results suggest that humans are successful on this task, with high agreement with the ground-truth annotation and the dataset label.



% \subsection{Models Evaluation}
% We evaluate several state-of-the-art vision-and-language models on this task. We note that currently there is no instruction-based vision-and-language model that has the potential to work better on this task.

% \paragraph{Setup.} We tested the following setups: (1) Image Captioning to instruction-based GPT3: An image captioning model, fine-tuned with OFA, provides an image caption that is fed to an instruction-based GPT3 model that transforms the caption into an explanation. An illustration of this setup is presented in Figure 3. We also added an "oracle" mode, where the instruction-based GPT3 receives the prompt that was used to create the image. To evaluate, we use human ratings and the automatic metric from the previous step (XYZ), which had the highest correlation with human ratings; (2) Visual Question Answering: We experimented with a state-of-the-art visual question answering model, fine-tuned with our dataset. We asked the model to predict the strangeness of the image and provide a justification. Since this model mostly provides short answers, we use rouge-1 recall and manual rating of its responses. Random examples of models predictions the evaluation metrics is presented in Appendix~\cref{appendix}, Section~\cref{model_predictions}.

% \input{figs_and_tables/table_two_step_model_evaluation.tex}
% \paragraph{Results.} Table~\cref{tab:two_step_model_evaluation} presents the results of the two-step model evaluation. It was found that all models performed poorly on this task, with performance ranging from 10\%-23\% according to all metrics. The oracle setup performed better than the other models, but still much lower than human performance. We observed that large language models such as GPT3 have difficulty understanding the subtle relations in our dataset, supporting the assertion that the task is challenging, even with a ``perfect'' image-captioning model. The gap between the image caption and prompt based results suggests a significant limitation in the image captioning model, which generates under-described captions. In these cases, the language model receives a non-strange caption and generates an incorrect explanation (e.g., when the image caption predicts ``A man holding a smartphone'' instead of ``Einstein holding a smartphone'', the instruction-based LM will always generate an incorrect explanation). In contrast, humans were able to succeed on the task even when only given the image and not the prompt. VQA results were much lower, at 0.05\%. The answers provided by these models are short and do not fit the expected explanation for the task. To summarize, we demonstrate that humans are able to succeed at the task of explaining what makes a given image strange, while current models struggle.






==> sections/99_evaluation.tex <==
We describe the evaluation setup used to assess the performance of both humans and models in \textit{identifying} weird images and \textbf{explaining} what makes them weird. By using this evaluation setup, we can obtain human-level performance results on these tasks.

\paragraph{Identifying weird vs.~normal images} Our objective is to investigate whether humans can accurately identify ``weird'' images. To achieve this, we collect 100 pairs of ``normal'' and ``weird'' image pairs as described in \cref{sec:image_generation}, and ask three human annotators to classify each image as either ``weird'' or ``normal''. We determine the final classification through a majority vote. Our results demonstrate that the annotators agree in their classification 92\% of the time and achieve complete agreement in 70\% of the cases. These results suggest that humans are capable of distinguishing between ``weird'' and ``normal'' images with high accuracy.

\paragraph{Evaluation of providing explanations} To retrieve both human and model performance, we design a single annotation task. We define the designer explanation as the target and include all of the explanations from both human and model baselines as candidate explanations. This includes the five human explanations collected in \cref{sec:image_generation} and the four model baselines described in \cref{sec:methods} and illustrated in \cref{fig:explanation_baselines}. We employ three annotators from Amazon Mechanical Turk (AMT) for each explanation and instruct them to select all explanations that have the same meaning as the designer explanation. The annotators achieve full agreement in XYZ\% of the cases, and we list the annotation results in the previous paragraphs. Overall, the annotation task show that models can provide explanations much better than current model baselines.
